Petri Automata

Kleene algebra axioms are complete with respect to both language models and binary relation models. In particular, two regular expressions recognise the same language if and only if they are universally equivalent in the model of binary relations. We consider Kleene allegories, i.e., Kleene algebras with two additional operations and a constant which are natural in binary relation models: intersection, converse, and the full relation. While regular languages are closed under those operations, the above characterisation breaks. Putting together a few results from the literature, we give a characterisation in terms of languages of directed and labelled graphs. By taking inspiration from Petri nets, we design a finite automata model, Petri automata, allowing to recognise such graphs. We prove a Kleene theorem for this automata model: the sets of graphs recognisable by Petri automata are precisely the sets of graphs definable through the extended regular expressions we consider. Petri automata allow us to obtain decidability of identity-free relational Kleene lattices, i.e., the equational theory generated by binary relations on the signature of regular expressions with intersection, but where one forbids unit. This restriction is used to ensure that the corresponding graphs are acyclic. We actually show that this decision problem is EXPSPACE-complete.

==> bits.tex <==


\section{From allegoric expressions to graph expressions}
\label{sec:from-alleg-expr}


\begin{lem}\label{lem:retypeprod}
  Let $G_1,G_2$ be a pair of TTSP graphs over $\sigdot$. We pose
  $G_k=\tuple{V_k,E_k}$ ($k\in\set{1,2}$), its source and sink being
  denoted respectively by $\iota_k$ and $o_k$. The following hold:
  \begin{align*}
    \retype{G_1}\cdot\retype{G_2}&=\retype{G_1\cdot G_2}\\
    \retype{G_1}\cap\retype{G_2}&=\retype{G_1\cap G_2}.
  \end{align*}
\end{lem}
\begin{center}
  \begin{tikzpicture}[xscale=2.5,yscale=1.5]
    \node (a) at (0,1) {TTSP$\tuple{\sigdot}\times$TTSP$\tuple{\sigdot}$};
    \node (b) at (2,1) {Graph$\tuple{\Sigma}\times$Graph$\tuple{\Sigma}$};
    \node (c) at (0,0) {TTSP$\tuple{\sigdot}$};
    \node (d) at (2,0) {Graph$\tuple{\Sigma}$};
    \edge(a)(b)[\retype{}\times\retype{}];
    \edge[below](c)(d)[\retype{}];
    \edge[left](a)(c)[\cdot/\cap];
    \edge[right](b)(d)[\cdot/\cap];
  \end{tikzpicture}
\end{center}
\begin{proof} 
  For the first equation, notice that every path (directed or not) in
  $G_1\cdot G_2$ that joins two vertices $i,j$ such that $i\in V_1$
  and $j\in V_2$ must visit the vertex $o_1/\iota_2$. This means that
  we can represent the equivalence classes of $\equiv_{G_1\cdot G_2}$
  as:
  \[\setcompr{[i]_{G_1}}{i\in V_1\setminus [o_1]_{G_1}}
    \cup\setcompr{[i]_{G_2}}{i\in V_2\setminus [\iota_2]_{G_2}}
    \cup\set{[o_1]_{G_1}\cup[\iota_2]_{G_2}}.\]
  % 
  This happens to be exactly the vertices of
  $\retype{G_1}\cdot\retype{G_2}$. We deduce easily from this the
  equality of the sets of edges and that of the inputs and outputs.

  The second equation is established in a similar manner. We
  notice here that every path in $G_1\cap G_2$ that goes from $V_1$
  to $V_2$ either visits $\iota_1/\iota_2$ or $o_1/o_2$. We may thus
  represent the equivalence classes of $\equiv_{G_1\cap G_2}$ as:
  \[\setcompr{[i]_{G_k}}{k\in\set{1,2},~i\in V_k\setminus
      \paren{[\iota_k]_{G_k}\cup [o_k]_{G_k}}}
    \cup\set{[\iota_1]_{G_1}\cup[\iota_2]_{G_2},
      [o_1]_{G_1}\cup[o_2]_{G_2}}.\]
  % 
  Again, this is the set of vertices of
  $\retype{G_1}\cap\retype{G_2}$, and it is immediate to check the
  equality from here.
\end{proof}
\begin{prop}\label{lem:al2gr}
  If $e\in\areg$ is in converse-normal form, $\grlang e = \retype{\Tr{\erasure e}}$.
\end{prop}
\begin{proof}
  We perform a structural induction on $e$. The base cases, namely
  $0,1,\top,a$ and $\conv a$, are immediate to check by merely
  unfolding the various definitions. The case of $e\cup f$ is not harder:
  \begin{align*}
    \retype{\Tr{\erasure {e\cup f}}} 
    & = \retype{\Tr{\erasure e\cup \erasure f}}
      = \retype{\Tr{\erasure e}\cup \Tr{\erasure f}}
      = \retype{\Tr{\erasure e}}\cup \retype{\Tr{\erasure f}}\\
    & = \grlang e\cup\grlang f = \grlang{e\cup f}
  \end{align*}
  For the case of the sequential and parallel products, as
  one would expect, Lemma~\ref{lem:retypeprod} will prove useful:
  \begin{align*}
    \grlang{e\cdot f}
    &=\setcompr{G\cdot G'}{\tuple{G,G'}\in \grlang e\times \grlang f}\\
    &=\setcompr{\retype{G}\cdot \retype{G'}}
      {\tuple{G,G'}\in \Tr {\erasure e}\times \Tr {\erasure f}}\\
    &=\setcompr{\retype{G\cdot G'}}
      {\tuple{G,G'}\in \Tr {\erasure e}\times \Tr {\erasure f}}\\
    &=\setcompr{\retype{G}}{G\in \Tr {\erasure {e\cdot f}}}
      =\retype{\Tr{\erasure{e\cdot f}}}\\
    \grlang{e\cap f}
    &=\setcompr{G\cap G'}{\tuple{G,G'}\in \grlang e\times \grlang f}\\
    &=\setcompr{\retype{G}\cap \retype{G'}}
      {\tuple{G,G'}\in \Tr {\erasure e}\times \Tr {\erasure f}}\\
    &=\setcompr{\retype{G\cap G'}}
      {\tuple{G,G'}\in \Tr {\erasure e}\times \Tr {\erasure f}}\\
    &=\setcompr{\retype{G}}{G\in \Tr {\erasure {e\cap f}}}
      =\retype{\Tr{\erasure{e\cap f}}}
  \end{align*}
  The case of $e^\star$ then follows simply from the cases of $\cup$
  and $\cdot$.
\end{proof}





\section{Comparing automata}
\label{sec:compare}

\subsection{Restriction}
\label{sec:restriction}


 This is because in combination with intersection, the
converse and identity operations operations introduce cycles in the
graphs associated to ground terms. Consider for instance the graphs
for $a\cap1$ and $a\cap \conv b$:
\begin{align*}
  G(a\cap1)&=
  \begin{tikzpicture}[baseline=(0.south)]
    \coordinate (loop) at (0,0.75);
    \node[above] (hop) at (loop) {$a$};
    \position (0) (0,0);
    \initst (0); \fnst (0);
    \draw[arc] (0) 
    to[above,out=135,in=180] (loop)
    to[out=0,in=55] (0);
  \end{tikzpicture}
  & G(a\cap \conv b)&=
  \begin{tikzpicture}[baseline=(0.south)]
    \position (0) (0,0);
    \position (1) (1.5,0);
    \initst (0);\fnst (1);
    \edge[above,out=20,in=160] (0) (1)[a];
    \edge[below,in=-20,out=-160] (1) (0)[b];
  \end{tikzpicture}
  \enspace.
\end{align*}

